Non-Stop & Non-Breakable Code Review Services in a Distributed System: Detecting Issues in Real Time

The two most significant bottlenecks in code merging are the build process and the unit tests. However, as the number of items to be checked in a code review increases, that code review becomes a bottleneck for code merging as well. Because of the dependency structure between code review services, an error in one service affects the entire service. As a result, whenever a service error occurs, it is crucial to have methods for determining which code review service has ultimately caused the error. With the goal of achieving a non-stop & non-breakable code review service, this paper describes an early error detection method along with a case study of the service.

==> memo/full-paper-plan.tex <==




#### works for submitting HCS Full paper

1. SR QT Lab / http://mosaic.sec.samsung.net/kms/qtlab.club
TEAM DOCS > 56. Code Review Innovation > 40. Docume... > CRB-Health-Check-System 


2. (ICSE-2022, Short paper) - Submitted on Oct-15-2021
* 저자명: 임근식, 박준배, 권용휘, 김철주 
* Title: Non–Stop & Non–Breakable Code Review Services in a Distributed System: Detecting Issues in Real Time
Anyone with this link can view this project (ICSE-2022, Short paper)
https://www.overleaf.com/read/zsdwzprkyjjt

3. Plan (ASE/FSE/ICSE, Industrial, Full paper)
* 저자명: 임근식, 박준배, 권용휘, (+ 김택수, 송윤기, 김형진), 김철주 
* Title: TBA (e.g., A Case Study for Non-stop Code Review Services at Samsung)





End of line. 
